Towards the understanding of heavy quarks hadronization: from leptonic to heavy-ion collisions

The formation of hadrons is a fundamental process in nature that can be investigated at particle colliders. As several recent findings demonstrate, with $\mathrm{e^+e^-}$ collisions as a "vacuum-like" reference at one extreme, and central nucleus--nucleus as a dense, extended-size system characterized by flow and local equilibrium at the opposite extreme, different collision systems offer a lever arm that can be exploited to probe with a range of heavy-flavour hadron species the onset of various hadronization processes. In this review, we present an overview of the theoretical and experimental developments. The focus is on open-heavy-flavour measurements. The comparison with model predictions and connections among the results in electron-positron, proton--proton, proton--nucleus, nucleus--nucleus collisions are discussed. After reviewing the current state, we suggest some prospects and future developments.

==> IntroductionB.tex <==
In the 1960s and 1970s it became clear that protons and neutrons of atomic nuclei, as well as many others in the zoo of particles that had been observed in cosmic-ray experiments and at accelerators were composite objects made of fundamental quarks. Quarks , the fundamental bricks of known matter. were com of atomic nuclei belong to a class of particles called hadrons, which are composite objects made of quarks, the fundamental bricks of known matter. Free quarks, not confined into hadrons, have never been observed in standard conditions of temperature and energy density. In Quantum Chromodynamic (QCD), the theory of strong interactions within the Standard Model of Particle Physics, this feature, called confinement, is expected by the from linearly rising trend of the attractive potential of quarks. However, at high energy densities, confinement is expected to disappear, leading to a transition to a quark-gluon plasma (QGP) state. The Early Universe was populated by free quarks and gluons up to about 10 microseconds after the Big Bang when hadron formation took place~\cite{}. The transition from a system of quarks to one of hadrons can be studied in laboratories: quarks represent the relevant degrees of freedom to understand particle production at particle colliders like the LHC at CERN. In collisions of protons or nuclei at the high LHC energies, one can model the production of the particles detected in the experimental apparatuses as a two-step process. First, an interaction (“hard scattering”) involving large energy transfer occurs over an extremely short timescale between the quarks of the colliding protons (or nuclei), resulting in the production of high-energy quarks. This initiates the second process, the hadronisation, in which the interaction between the existing quarks causes the production of additional quarks and ultimately the formation of hadrons. When nuclei are collided at high energy the quark and gluon density and the system size are large enough to allow for a QGP phase with properties similar to that of the Early Universe, and in which quarks and gluons interact several times, delaying hadron formation.

Though quantum chromodynamic (QCD), the fundamental theory of strong interactions, was formulated about 50 years ago, the theoretical understanding of the hadronisation dynamics is extremely challenging, because the processes involved cannot be calculated with perturbative techniques from first principles. Therefore, a modelling of the process based on first-principle QCD, Lattice QCD calculations, as well as phenomenological considerations is necessary.

In order to study the production of hadronic states in high-energy collisions, we use what are known as “event generators”, which use numerical simulations to provide the most general and detailed descriptions of hadronic production. Though several features emerging from experimental observations are described by event generators, a comprehensive and satisfactory description is yet missing. In particular, what emerged in recent years are unexpected differences between hadron production in high-energy e+e- collisions and in proton-proton collisions.  The ALICE experiment observed that the ratio of the production rate of baryons (i.e. hadrons containing three quarks, as protons and neutrons) and mesons (i.e. hadrons containing two quarks, as the pion, the lighter hadron) is significantly larger in proton-proton collisions with respect to e+e- collisions, contrary to expectations. The difference is remarkably large when heavy hadrons containing at least one heavy quark (“charm” or “beauty” quarks, which have masses around 1.5 and 5 times larger than the proton mass respectively) are considered, as observed by both the ALICE and LHCb experiments. Heavy quarks cover a special role for the understanding of hadronisation: because of their large mass, they can be produced only in processes with larger energy transfer, thus only in hard-scattering processes at the beginning of collision, well before hadronisation takes place. The rate of these processes can be calculated from first principle in QCD. This makes them ideal “calibrated” probes of the hadronisation process, during which they get “attached” to other quarks (mainly light “up”, “down”, and “strange” quarks) or pairs of quarks (diquarks), which can either be already present in the system or be produced during the same hadronisation process. By comparing the production rates and the kinematic properties of several massive hadrons with different quark content and quantum numbers, a window can be open on the microscopic processes involved during hadronisation, on how light quarks and diquarks are produced and how they correlate and combine to ultimately form hadrons. 

